Bandwidth Optimal Pipeline Schedule for Collective Communication

We present a strongly polynomial-time algorithm to generate bandwidth optimal allgather/reduce-scatter on any network topology, with or without switches. Our algorithm constructs pipeline schedules achieving provably the best possible bandwidth performance on a given topology. To provide a universal solution, we model the network topology as a directed graph with heterogeneous link capacities and switches directly as vertices in the graph representation. The algorithm is strongly polynomial-time with respect to the topology size. This work heavily relies on previous graph theory work on edge-disjoint spanning trees and edge splitting. While we focus on allgather, the methods in this paper can be easily extended to generate schedules for reduce, broadcast, reduce-scatter, and allreduce.

==> related_work.tex <==
\section{Related Work}

In previous literature, Blink~\cite{blink} is the closest to our work. Blink uses packing of spanning trees, which is also the foundation of our work. However, Blink only considers broadcast and offers no proof of optimality. Blink asserts that many-to-many operations like allreduce can be achieved by reduce+broadcast, but we have shown in \S\ref{sec:allreduce} that such an approach has worse bandwidth performance than reduce-scatter followed by allgather. Furthermore, Blink's construction does not consider switch nodes.\\

There are many other works that try to generate optimal reduce-scatter/allgather/allreduce schedule for a given network topology. BlueConnect~\cite{cho2019blueconnect} optimizes collective for switch-based Clos-like topologies, but it only considers tree network topologies. SCCL~\cite{SCCL} and TACCL~\cite{taccl} use SMT-solver and MILP to search for optimal schedules. Their scalabilities are limited due to the NP-hardness of SMT-solver and MILP. 

==> spanning_tree_backup.tex <==
\subsection{Spanning Tree Construction}\label{sec:constructtree}

\begin{algorithm}[tb]
    \caption{Batched Spanning Tree Construction}
    \label{algo:construct}
    \SetAlgoLined
    \DontPrintSemicolon
    \KwIn{Integer-capacity Eulerian digraph $G^*=(V_c,E^*)$ and $k\in\N$.}
    \KwOut{Edge-disjoint Spanning Trees $\{T_{u,i}\}_{u\in V_c,i\in [k]}$ with $T_{u,i}$ rooted at $u$ and $\cV(T_{u,i})=V_c$.}
    \Begin{
        Initialize $T_{u,1}=\emptyset$, $R_{u,1}=\{u\}$, and $c_{u,1}=k$ for all $u\in V_c$.\;
        $D'\leftarrow G^*$\;
        \While{\normalfont there exists $R_{w,j}\neq V_c$}{
            \While{\normalfont $R_{w,j}\neq V_c$}{
                Pick an edge $(x,y)$ in $D'$ that $x\in R_{w,j},y\notin R_{w,j}$.\;
                Binary search the maximum $c$ satisfying $c\leq c_{w,j}$, $c\leq c(x,y;D')$, and $F(x,y;\overline{D'})\geq|V_c|k$ with $(x,s_{w,j})$ having a capacity of $c_{w,j}-c$ in $\overline{D'}$.\;
                \lIf{\normalfont $c=0$}{\textbf{continue}}
                \If{\normalfont $c<c_{w,j}$}{
                    Create a new batch $T_{w,h}=T_{w,j}$, $R_{w,h}=R_{w,j}$, and $c_{w,h}=c_{w,j}-c$.\;
                    $c_{w,j}\leftarrow c$\;
                }
                $T_{w,j}\leftarrow T_{w,j}+(x,y)$\;
                $R_{w,j}\leftarrow R_{w,j}+y$\;
                Remove $c$ capacity of $(x,y)$ from $D'$. Remove $(x,y)$ if its capacity reaches 0.\;
            }
        }
    }
\end{algorithm}

We use the algorithm proposed by Tarjan~\cite{tarjan} to construct edge-disjoint spanning trees in $G^*=(V_c,E^*)$ but with some modifications. The modifications are targeted to make the construction faster when $k$, the number of spanning trees per compute node, is large. Although this does not obviate the runtime dependency on $k$, the modified algorithm is significantly faster in practice.\\

We start by showing the existence of spanning trees with the following theorem in Tarjan~\cite{tarjan}. The theorem was originally proven by Edmonds~\cite{edmonds}.
\begin{restatable}[Tarjan~\cite{tarjan}]{theorem}{thmtarjan}\label{thm:tarjan}
    For any integer-capacity digraph $D=(V,E)$ and any sets $R_i\subseteq V$, $i\in[k]$, there exist $k$ edge-disjoint spanning out-trees $T_i$, $i\in[k]$, rooted respectively at $R_i$, if and only if for every $S\neq V$,   
    \begin{equation}\label{eq:tjcondition}
        c(S,\bar{S};D)\geq|\{i\ |\ R_i\subseteq S\}|.
    \end{equation}
\end{restatable}
A spanning out-tree is \textit{rooted at $R_i$} if for every $v\in V-R_i$, there is exactly one directed path from a vertex in $R_i$ to $v$ within the out-tree subgraph. To see there exists a family of edge-disjoint spanning out-trees $\{T_{u,i}\}_{u\in V_c,i\in[k]}$ in $G^*$, observe that each $T_{u,i}$ is rooted at $R_{u,i}=\{u\}$, so $|\{(u,i)\ |\ R_{u,i}\subseteq S\}|=|S|k$ for any $S\subset V_c,S\neq V_c$. We show the following theorem:
\begin{restatable}{theorem}{thminitialexist}\label{thm:initialexist}
    Given integer-capacity digraph $D=(V_c,E)$ and $k\in\N$, $c(S,\bar{S};D)\geq|S|k$ for all $S\subset V_c,S\neq V_c$ if and only if $\min_{v\in V_c}F(s,v;\vec{D}_k)\geq|V_c|k$.
\end{restatable}
Since we ensured $\min_{v\in V_c}F(s,v;\vec{G}^*_k)\geq|V_c|k$, condition (\ref{eq:tjcondition}) is satisfied. Spanning tree construction essentially involves iteratively expanding each $R_{u,i}$ from $\{u\}$ to $V_c$, while maintaining condition (\ref{eq:tjcondition}). Let $T_{u,i}$ be the $i$-th tree rooted at $u$ currently under construction, and let $D-\bigcup_{u,i}T_{u,i}$ be the subgraph of $D$ with all edges in $\bigcup_{u,i}T_{u,i}$ removed. We should remind readers that we are thinking of capacity as the number of multiedges. Thus, $D-\bigcup_{u,i}T_{u,i}$ is decreasing an edge $e$ by capacity one whenever $e$ is in some $T_{u,i}$ instead of removing $e$ completely. In Tarjan~\cite{tarjan}, the following lemma has been shown:
\begin{restatable}[Tarjan~\cite{tarjan}]{lemma}{lmtarjan}\label{lm:tarjan}
    Given an integer-capacity digraph $D=(V_c,E)$ and $R_{u,i}=\cV(T_{u,i})$, $u\in V_c,i\in[k]$, such that (\ref{eq:tjcondition}) holds for all $S\neq V_c$. For any $R_{w,j}\neq V_c$, there is an edge $(x,y)$ in $D-\bigcup_{u,i}T_{u,i}$ such that $x\in R_{w,j}$, $y\notin R_{w,j}$, and for all $S$, $x\in S,y\notin S$ imply
    \[
        \textstyle c(S,\bar{S};D-\bigcup_{u,i}T_{u,i})\geq|\{(u,i)\ |\ (u,i)\neq(w,j),R_{u,i}\subseteq S\}|+1.
    \]
\end{restatable}
Obviously, adding $(x,y)$ to $T_{w,j}$ and consequently $y$ to $R_{w,j}$ does not violate condition (\ref{eq:tjcondition}). Thus, for each $T_{u,i}$, we can continuously pick such edge $(x,y)$ to include more vertices until $R_{u,i}=V_c$. This is exactly the algorithm described in Tarjan~\cite{tarjan}.\\

The process of adding $(x,y)$ to $T_{u,i}$ in our context is to decrease the capacity of $(x,y)$ in $D-\bigcup_{u,i}T_{u,i}$ by one and add one capacity of $(x,y)$ to $T_{u,i}$. As in \S\ref{sec:edgesplit}, this is inefficient when the number of trees we need to construct is large. Here, we give a way to add one edge to multiple trees at once. Let $(x,y)$ be an edge in $D-\bigcup_{u,i}T_{u,i}$, and let $\cT$ be a subcollection of $\{T_{u,i}\}_{u\in V_c,i\in[k]}$ such that $x\in\cV(T),y\notin\cV(T)$ for all $T\in\cT$. For the simplicity of notation, let $D-\bigcup_{u,i}T_{u,i}$ be $D'$. We construct a flow network $\overline{D'}$ that (a) a node $s_{u,i}$ is added for each $T_{u,i}\notin\cT$, (b) connect $x$ to each $s_{u,i}$ with capacity 1, and (c) connect each $s_{u,i}$ to every vertex in $R_{u,i}=\cV(T_{u,i})$ with capacity $\infty$. We have the following theorem:
\begin{restatable}{theorem}{thmmultipletree}\label{thm:multipletree}
    $F(x,y;\overline{D'})\geq|V_c|k$ if and only if for all $S$, $x\in S,y\notin S$ imply
    \begin{equation}\label{eq:multipletree}
        c(S,\bar{S};D')\geq|\{(u,i)\ |\ T_{u,i}\notin\cT,R_{u,i}\subseteq S\}|+|\cT|.
    \end{equation}
\end{restatable}
In practice, we construct trees in batches to speed up construction. At the beginning, each $u\in V_c$ has a batch $T_{u,1}=\emptyset,R_{u,1}=\{u\}$ that delivers $k$ capacity. Given a $T_{u,i}$ with $c_{u,i}$ capacity, we use theorem \ref{thm:multipletree} to test if we can add $c_{u,i}$ capacity of $(x,y)$ to $T_{u,i}$. If not, suppose the maximum capacity of $(x,y)$ that can be added to $T_{u,i}$ is $c>0$. In this case, we split $T_{u,i}$ into two batches, $T_{u,j}$ and $T_{u,h}$, where $T_{u,j}$ and $T_{u,h}$ deliver capacities of $c$ and $c_{u,i}-c$ respectively. Finally, we add $c$ capacity of $(x,y)$ to $T_{u,j}$, and the algorithm continues. In addition, when constructing $\overline{D'}$, we assign a capacity of $c_{u,i}$ to edge $(x,s_{u,i})$. The pseudocode is provided in Algorithm \ref{algo:construct}. \\

After spanning tree construction, we have spanning trees $\{T_{u,i}\}_{u\in V_c,i\in [k]}$ in $G^*$. Each of the edge $(u,v)$ in $T_{u,i}$ may correspond to a path $u\to w_1\to\dots\to w_n\to v$ in $G$ with $w_1,\dots,w_n$ being switch nodes. In other words, edges in $T_{u,i}$ only specify the source and destination of send/recv between compute nodes. Thus, one needs to use the \emap in algorithm \ref{algo:removeswitch} to recover the paths in $G$. For any edge $(u,t)$ in $G^*$, $\emap[(u,t)][w]$ denotes the amount of capacity from $u$ to $t$ that is going through $(u,w),(w,t)$. It should be noted that \emap may be recursive, meaning that $(u,w),(w,t)$ may also go through some other switches. Because each capacity of $(u,t)$ corresponds to one capacity of a path from $u$ to $t$ in $G$, the resulting pipeline schedule in $G$ has the same performance in $G^*$, achieving the optimal bandwidth performance in $G$. \\

In figure \ref{fig:states}'s example, we construct a spanning tree like \ref{fig:topo_split_tree} for each of the compute node. By reversing the edge splitting with \emap, the spanning tree becomes the pipeline schedule in \ref{fig:topo_tree2}. Note that the corresponding pipeline schedule of a spanning tree in $G^*$ is not necessarily a tree in $G$. For example, the pipeline schedule in \ref{fig:topo_tree2} visits switches $v_1^s,v_2^s$ multiple times. To obtain a pipeline allgather with optimal bandwidth runtime $(M/N)(4/4b)$, one can apply the similar pipeline schedule for each of the compute nodes in \ref{fig:topo_tree2}.\\

One may be tempted to devise a way to construct spanning trees with low heights. This has numerous benefits such as lower latency at small data sizes and better convergence of pipeline schedule towards bandwidth optimality. Although there is indeed potential progress to be made in this direction, constructing edge-disjoint spanning trees of minimum height has been proven to be NP-complete~\cite{npcomplete}.

\lmtarjan*
\thmmultipletree*
\begin{proof}
    $\Rightarrow$: Suppose there exists $S$ that (\ref{eq:multipletree}) is violated. Consider the $x$-$y$ cut $(A,\bar{A})$ in $\overline{D'}$ such that $A=S\cup\{s_{u,i}\ |\ T_{u,i}\notin\cT,R_{u,i}\subseteq S\}$. It follows that
    \begin{align*}
        c(A,\bar{A};\overline{D'})
        &=c(S,\bar{A};\overline{D'})+\sum_{T_{u,i}\notin\cT,R_{u,i}\not\subseteq S}c(x,s_{u,i};\overline{D'})\\
        &=c(S,\bar{S};D')+|\{s_{u,i}\ |\ T_{u,i}\notin\cT,R_{u,i}\not\subseteq S\}|\\
        &<|\{(u,i)\ |\ T_{u,i}\notin\cT,R_{u,i}\subseteq S\}|+|\cT|+|\{s_{u,i}\ |\ T_{u,i}\notin\cT,R_{u,i}\not\subseteq S\}|\\
        &=|V_c|k.
    \end{align*}
    By min-cut theorem, $F(x,y;\overline{D'})\leq c(A,\bar{A};\overline{D'})<|V_c|k$\\
    
    $\Leftarrow$: Suppose $F(x,y;\overline{D'})<|V_c|k$. Let $(A,\bar{A})$ be the $x$-$y$ cut that $c(A,\bar{A};\overline{D'})<|V_c|k$. Let $S=A\cap V_c$. It follows that
    \begin{align*}
        c(S,\bar{S};D')
        &=c(S,\bar{A};\overline{D'})\\
        &\leq c(A,\bar{A};\overline{D'})-|\{s_{u,i}\ |\ T_{u,i}\notin\cT,R_{u,i}\not\subseteq S\}|\\
        &<|V_c|k-|\{s_{u,i}\ |\ T_{u,i}\notin\cT,R_{u,i}\not\subseteq S\}|\\
        &=|\{(u,i)\ |\ T_{u,i}\notin\cT,R_{u,i}\subseteq S\}|+|\cT|.
    \end{align*}
    The first inequality follows the fact that for any $R_{u,i}\not\subseteq S$, edge $(x,s_{u,i})$ crosses the cut $(A,\bar{A})$; otherwise, there exists $v\in R_{u,i}-S$ that $\infty$-capacity edge $(s_{u,i},v)$ crosses the cut. Thus, $c(A-S,\bar{A};\overline{D'})\geq|\{s_{u,i}\ |\ T_{u,i}\notin\cT,R_{u,i}\not\subseteq S\}|$.
\end{proof}
